A Closer Look at Personalized Fine-Tuning in Heterogeneous Federated Learning

Federated Learning (FL) enables decentralized, privacy-preserving model training but struggles to balance global generalization and local personalization due to non-identical data distributions across clients. Personalized Fine-Tuning (PFT), a popular post-hoc solution, fine-tunes the final global model locally but often overfits to skewed client distributions or fails under domain shifts. We propose adapting Linear Probing followed by full Fine-Tuning (LP-FT), a principled centralized strategy for alleviating feature distortion (Kumar et al., 2022), to the FL setting. Through systematic evaluation across seven datasets and six PFT variants, we demonstrate LP-FT's superiority in balancing personalization and generalization. Our analysis uncovers federated feature distortion, a phenomenon where local fine-tuning destabilizes globally learned features, and theoretically characterizes how LP-FT mitigates this via phased parameter updates. We further establish conditions (e.g., partial feature overlap, covariate-concept shift) under which LP-FT outperforms standard fine-tuning, offering actionable guidelines for deploying robust personalization in FL.

==> table/PFL.tex <==
\begin{table}[H]
  \centering
  % \vspace{-20pt} % Adjust vertical space as needed
  % \resizebox{0.42\textwidth}{!}{
  \begin{tabular}{>{\bfseries}lccc}
    \toprule
    PFL Method & Local Acc. ($\uparrow$) & Global Acc. ($\uparrow$) & Avg. Acc. \\
    \midrule
    % FedBabu & 92.16 & 81.47 & 80.10 \\
    FedBN~\citep{DBLP:conf/iclr/LiJZKD21} & 88.68 & 61.35 & 61.00 \\
    PerAvg~\citep{DBLP:conf/nips/0001MO20} & 87.06 & 67.26 & 66.66 \\
    FedNova~\citep{DBLP:conf/nips/WangLLJP20} & 88.68 & 54.26 & 53.41 \\
    FedRep~\citep{DBLP:conf/icml/CollinsHMS21} & 86.94 & 52.99 & 52.57 \\
    FedSoup~\citep{DBLP:conf/miccai/ChenJDWL23} & 90.30 & 75.62 & 75.21 \\
    FedSelect~\cite{DBLP:conf/cvpr/TamirisaXBZAS24} & 90.93 & \textbf{86.15} & \textbf{82.90} \\
    
    LP-FT & \textbf{93.03} & 82.46 & 82.17 \\

    \bottomrule
  \end{tabular}
  % }
  \caption{Different PFL Methods on CelebA.}
  \label{tab:app_pfl}
  \vspace{-4mm} % Adjust vertical space as needed
\end{table}

